Triplet Reconstruction and all other Phylogenetic CSPs are Approximation Resistant

We study the natural problem of Triplet Reconstruction (also Rooted Triplets Consistency or Triplet Clustering), originally motivated in computational biology and relational databases (Aho, Sagiv, Szymanski, and Ullman, 1981): given $n$ points, we want to embed them onto the $n$ leaves of a rooted binary tree (a hierarchical clustering or ultrametric embedding) such that a given set of $m$ triplet constraints is satisfied. Triplet $ij|k$ indicates that ``$i, j$ are more closely related to each other than to $k$'' and a tree satisfies $ij|k$ if $d(i,j)$ is the smallest among the 3 distances. Aho et al. (1981) gave an elegant efficient algorithm to find a tree respecting all constraints (if it exists) and it is easy to see that a random binary tree is a 1/3-approximation. Unfortunately, despite more than four decades of research, no better approximation is known. Our main theorem--which captures Triplet Reconstruction as a special case--is a general hardness of approximation result about Constraint Satisfaction Problems (CSPs) over infinite domains (the variables are mapped to any of the $n$ leaves of a tree). Specifically, we prove, under Unique Games (Khot, 2002), that Triplet Reconstruction and more generally, every CSP over hierarchies is approximation resistant (there is no polynomial-time algorithm that does asymptotically better than a biased random assignment). This settles the approximability for many interesting Subtree or Supertree Aggregation Problems. More broadly, our result significantly extends the list of approximation resistant predicates and is a generalization of Guruswami, Hastad, Manokaran, Raghavendra, and Charikar (2011), who showed that ordering CSPs are approximation resistant. The main challenge in our analyses stems from the fact that trees have topology which is what determines whether a given triplet constraint on the leaves is satisfied or not.

==> figures/triplets-to-quartets-fig.tex <==
%NOT USED AFTER ALL

 \tikzset{
every tree node/.style={minimum width=1em,draw,circle, fill=gray!50},
%%
blank/.style={draw=none},
edge from parent/.style={draw,edge from parent path={(\tikzparentnode) -- (\tikzchildnode)}},
level distance=1cm,
}
\tikzset{ELS/.style = {% Edge Label Style
              pos=0.5, sloped, node font=\footnotesize, text=blue,
              inner sep=2pt},
        }
   
   \begin{tikzpicture}
\Tree
[.\node[fill=black, text=white]{{}}; 
[.\node[fill=gray!90, text=white]{{}}; 
[.\node[fill=teal, text=white]{{$a$}}; ] 
[.\node[fill=teal, text=white]{{$b$}}; ]] [.\node[fill=teal, text=white]{{$c$}}; ]]
]
\end{tikzpicture}
%\vspace{-0.5cm}
%$\iff$
 \centering
    \begin{forest}
for tree = {
% node style
    circle,
    draw=black,
    line width=0.1mm,
    fill=teal,
    minimum size=1mm,
tikz/every label/.style = {font=\sffamily\bfseries},
% tree style
    edge = {thin},
    l sep=6mm,
    s sep=7mm,
EL/.style={if n=1{edge label={node[ELS, anchor=south]{}}}
                 {edge label={node[ELS, anchor=north]{}}}}
           }
% tree body code
[,coordinate, label={[ELS]}
    [ , fill=black, text=white,
        %%%%    settings for the right branch
        for tree={grow'=east}, 
        before computing xy={l=0, s=+7mm},
        %%%%
       [,label=right:$c$,  EL=2]
       [,label=right:$\gamma$, EL=0]
    ]
    [ , fill=gray,
        %%%%    settings for the left branch
        for tree={grow=west},
        before computing xy={l=0, s=-7mm},
        %%%%
        [,label=left:$a$,  EL=1]
        [,label=left:$b$, EL=2]
    ]
]
    \end{forest}
  
   


==> paper/further.tex <==
\section{Further Related Work}
\paragraph{Beyond Triplets and Quartets.} Inferring an evolutionary tree from triplets (\textsc{MaxRTC}) or quartets (\textsc{MaxUQC}) are just two simple examples of a broader set of methods called ``consensus tree'' or ``supertree'' methods~\citep*{adams1972consensus,sanderson1998phylogenetic,steel2000simple}. Briefly, the goal of such methods is to aggregate local information about $n$ species, presented as phylogenies with overlapping sets of leaves and to output a single phylogenetic tree that summarizes the branching structure of collected information. Such methods have a variety of applications~\citep*{bryant2003classifica,brodal2013efficient} and as a result, they have also been heavily studied in computer science~\citep*{henzinger1999constructing,farach1995agreement,kannan1998computing,ng1996reconstruction,semple2000supertree,jansson2016improved}. %should we say that triplets generalizes the moseley wang objective?
\vnote{cite Moses: Fitting Tree Metrics, Cohen-Addad's follow-up recent}
More technically distant
analogs of these stability conditions (but with similar motivation) were proposed by [1, 19, 37];
Thorup fitting metrics old paper as well (On the Approximability of Numerical Taxonomy
(Fitting Distances by Tree Metrics))


==> paper/old_abstract.tex <==
\thispagestyle{empty}
\begin{abstract}
%FIX 
%related work
%examples&counterexamples, 
%prelims
\vnote{other title? Infinite domain CSPs?}

%Subgraph counting is a fundamental problem that spans many areas in computer science: database theory, logic, network science, data mining, and complexity theory. Given a large input graph G and a small pattern graph H, we wish to count the number of occurrences of H in G. In recent times, there has been a resurgence on using an old (maybe overlooked?) technique of orienting the edges of G and H, and then using a combination of brute-force enumeration and indexing. These orientation techniques appear to give the best of both worlds. There is a rigorous theoretical explanation behind these techniques, and they also have excellent empirical behavior (on large real-world graphs). Time and again, graph orientations help solve subgraph counting problems in various computational models, be it sampling, streaming, distributed, etc. In this paper, we give some short vignettes on how the orientation technique solves a variety of algorithmic problems.


%A central problem in computer science is to count or enumerate the occurrences of a small pattern graph H in a large input graph G. The applications of graph pattern counts occur across numerous scientific areas, including logic, biology, statistical physics, database theory, social sciences, machine learning, and network science [36, 13, 17, 12, 24, 9, 30, 55, 48, 21, 47]. The tutorial [51] has more details on applications. A rich and deep theory has emerged from the study of graph pattern counting [41, 14, 32, 19, 42, 2, 18, 48, 49].

%The basic problem of triplet reconstruction...


We study the approximability of a broad class of computational problems---originally motivated in  evolutionary biology and phylogenetic reconstruction---concerning the aggregation of potentially inconsistent (local) information about $n$ items of interest, and we present optimal hardness of approximation results under the Unique Games Conjecture.

The class of problems studied here can be described as Constraint Satisfaction Problems (CSPs) over \textit{infinite} domains, where instead of values $\{0,1\}$ or a fixed-size domain, the variables can be mapped to any of the $n$ leaves of a phylogenetic tree. The \textit{topology} of the tree then determines whether a given constraint on the variables is satisfied or not, and the resulting CSPs are called \textit{Phylogenetic CSPs}. Prominent examples of Phylogenetic CSPs with a long history and applications in various disciplines include:


\begin{itemize}
    \item \textbf{Triplet Reconstruction:} A triplet constraint $ij|k$ indicates that ``items $i,j$ are more similar to each other than to $k$.'' Given $m$ triplets, we would like to construct a hierarchical clustering on the $n$ items, that respects constraints as much as possible, i.e., the ancestry relation in the hierarchy places $i,j$ in some cluster that does not contain $k$. This gives rise to the well-studied ``Rooted Triplets Consistency'' problem in computational biology.
    \item \textbf{Quartet Reconstruction:} Similarly to the triplet reconstruction, biologists often perform experiments on quadruples of points $a,b,c,d$ and want to find an unrooted phylogenetic tree that best reflects the collected information. This gives rise to the well-studied ``Unrooted Quartet Consistency'' problem in phylogenetics.
    \item \textbf{Subtree Aggregation (Forbidden or Desired):} More generally, allowing for conjunctions (logical $\land$) or disjunctions (logical $\lor$) between constraints, a series of well-studied computational problems arises (``supertree'' or ``subtree'' aggregation methods). For example, $ij|k \lor ik|j$ captures the \textit{forbidden} triplets problem, that forbids triplets $jk|i$ from the final hierarchy.
\end{itemize}

Despite more than four decades of research, the basic question of maximizing the number of satisfied constraints is not well-understood. The current best approximation is achieved by outputting a \textit{random} tree or by a greedy construction. For example, for the case of triplets, a $\tfrac13$ ratio is achieved by a random tree since there are only 3 distinct triplets $ij|k,ik|j,jk|i$ (each appears with probability $\tfrac13$). 

Our main result is that \textit{every} Phylogenetic CSP is \textit{approximation resistant}, i.e., there is no polynomial-time algorithm that does asymptotically better than a (biased) random assignment. This is a generalization of the results in~\citet*{GHMRC11}, who showed that \textit{ordering} CSPs are approximation resistant (e.g., Max Acyclic Subgraph and Betweenness). 

%%KM: Let's move the following
%%to introduction, otherwise
%%it looks a bit out of place
%%Our hardness reductions build upon the gap instances used in their work; here however, we need to overcome several technical difficulties stemming from the fact that trees have topology (in contrast to permutations, which can be thought of as a special case of  ``flat'' trees) and this underlying topology determines if a constraint is satisfied or not.

%A common characteristic of  For all these combinatorial optimization problems, the current best is RANDOM: simply output

%Having access to such local information is used in crowdsourcing, recommendation and psychology since humans are good at providing comparisons rather than absolute scores. Despite four decades of research, a random solution is best we know, and we show that this is indeed optimal under UGC. Is this a coincidence?

%triplet in Aho databases theory
%exact is understood via the algebraic method by algebraic/logic community, we extend approximability, main challenges, we separate triplets quartets but questions makes sense more generally

%A popular special case of Phylogenetic CSPs is \textit{Triplet Reconstruction}, which has played an important role across several domains, including relational databases, crowdsourcing, and psychology: given a ground set of $n$ elements and $m$ triplets of the form $ab|c$,  we want to find a hierarchical clustering $T$
%(e.g., rooted, binary, unordered tree)
%on $n$ leaves, such that $T$ satisfies all or as many of the triplets as possible, in the sense that in the hierarchical decomposition induced by $T$, the lowest common ancestor of $a,b$ is a proper descendant of the lowest common ancestor of $a,c$. In 1981, motivated by applications in relational database theory, ~\cite{aho1981inferring} showed that in the complete case (i.e., all constraints are satisfiable), a top-down method will find a tree $T$ satisfying all triplets. However, despite four decades of research, the optimization problem of maximizing the number of satisfied triplets only has a trivial $\tfrac13$-approximation, achieved by a random tree or by a greedy construction. Similarly, for other related problems like \textit{Quartet Reconstruction} (where constraints are specified on quadruples $ab|cd$ instead of triplets), the current best approximation is also achieved by a random tree.

%In this paper, we systematically investigate whether this is a coincidence or whether there are  computational barriers that prevent us from beating these trivial baselines. Our first main result is to show that, assuming the Unique Games Conjecture,  Triplet Reconstruction and Quartet Reconstruction are \textit{approximation resistant} (i.e., the random assignment is best possible). Our second main result, which turns out to be the most challenging, is to prove that every phylogenetic CSP is approximation resistant. This is a strengthening of the results in~\citet*{GHMRC11}, who showed that \textit{ordering} CSPs are approximation resistant, and our hardness reductions build upon the gap instances used in~\cite{GHMRC11}. Here, however, we need to overcome several technical difficulties stemming from the fact that trees have topology (in contrast to permutations, which can be thought of as a special case of  ``flat'' trees) and the underlying topology determines if a constraint is violated or not.

%mention optimal leaf ordering for ordered trees where left right matters!




%Our starting motivation was a basic question about the following triplet reconstruction problem on trees: given a ground set of $n$ elements and $m$ (triplet) constraints of the form $ab|c$, find a rooted, binary, unordered tree $T$ on $n$ leaves, such that $T$ satisfies as many of the triplets as possible, in the sense that in the hierarchical decomposition induced by $T$, the lowest common ancestor of $a,b$ is a proper descendant of the lowest common ancestor of $a,c$. In the context of phylogenetics, this is the Rooted Triplets Consistency problem, which essentially asks how do we aggregate local information about triples of species $a,b,c$ into a global hierarchy.

%Since its introduction in 1981 by~\citeauthor{aho1981inferring}, Rooted Triplets Consistency has played an important role across several domains, like database theory, crowdsourcing, and psychology. However, the best approximation known so far is to output random tree on $n$ leaves, which obtains a $\tfrac13$-approximation, simply because there are  three distinct triplets on $a,b,c$, namely $ab|c,ac|b,bc|a$ and the random tree will satisfy each with probability $\tfrac13$. 

%Thus, every permutation CSP of arity up to 3 resists approximation beyond the trivial random ordering threshold. In contrast, for Boolean CSPs, there are both approximation resistant and non-trivially approximable CSPs of arity 3.

\end{abstract}


%Includes many problems in hierarchical clustering

%and our results address open questions for many popular methods such as rooted triplets
%consistency, unrooted quartets consistency, forbidden subtree problems and many
%other problems studied in the bioinformatics literature. Prominent examples: 
